InfinityGAN: Towards Infinite-Pixel Image Synthesis

We present a novel framework, InfinityGAN, for arbitrary-sized image generation. The task is associated with several key challenges. First, scaling existing models to an arbitrarily large image size is resource-constrained, in terms of both computation and availability of large-field-of-view training data. InfinityGAN trains and infers in a seamless patch-by-patch manner with low computational resources. Second, large images should be locally and globally consistent, avoid repetitive patterns, and look realistic. To address these, InfinityGAN disentangles global appearances, local structures, and textures. With this formulation, we can generate images with spatial size and level of details not attainable before. Experimental evaluation validates that InfinityGAN generates images with superior realism compared to baselines and features parallelizable inference. Finally, we show several applications unlocked by our approach, such as spatial style fusion, multi-modal outpainting, and image inbetweening. All applications can be operated with arbitrary input and output sizes. Please find the full version of the paper at https://openreview.net/forum?id=ufGMqIM0a4b .

==> codes/forward.tex <==
\begin{minted}[
    bgcolor=backcolor,
    frame=lines,
    framesep=1mm,
    % baselinestretch=1.2,
    fontsize=\tiny,
    linenos,
    numbers=left,
    % baselinestretch=.93,
    breaklines
]{python}
import torch
import torch.nn.functional as F

def forward(self, feature, style):
    """
    feature: Feature with shape (B, C1, H, W)
    style  : Single style with shape (B, C2)
    """
    batch, in_c, in_h, in_w = feature.shape

    
    # Hyperparameters
    k = self.kernel_size # Conv kernel size
    out_c = self.out_c   # Expected output channel
    rmpad = k // 2       # Zero-padding removal
    
    # Weight scaling (StyleGAN2)
    # Shape:
    # (1, ) * (out_c, in_c, k, k)
    # => (out_c, in_c, k, k)
    weight = self.scale * self.weight

    # Weight modulation (StyleGAN2)
    style = self.modulation(style)
    style = style.view(batch, 1, in_c, 1, 1)
    # Shape:
    # (1, out_c, in_c, k, k) * (batch, 1, in_c, 1, 1)
    # => (batch, out_c, in_c, k, k)
    weight = weight.unsqueeze(0) * style





    # Weight demodulation (StyleGAN2)
    demod = torch.rsqrt(
        weight.pow(2).sum([2,3,4]))
    weight *= demod.view(batch, out_c, 1, 1, 1)
    










    # Convolution
    feature = feature.view(1, batch*in_h, in_h, in_w)
    if self.upsample:
        weight = weight.view(batch, out_c, in_c, k, k)
        weight = weight.transpose(1, 2).reshape(
            batch*in_c, out_c, k, k)
        out = F.conv_transpose2d(
            feature, weight, 
            padding=0, stride=2, groups=batch)

        # Clipping zero padding (ConvT special case)
        out = out[:, :, rmpad:-rmpad, rmpad:-rmpad]








        out = self.blur(out) # StyleGAN2 Gaussian blur
    else:
        weight = weight.view(batch*out_c, in_c, k, k)
        out = F.conv2d(
            feature, weight, padding=0, groups=batch)
    
    # Recover batch-channel shape due to grouping
    _, _, out_h, out_w = out.shape
    out = out.view(batch, out_c, out_h, out_w)

    return out
\end{minted}

==> codes/fused_forward.tex <==
\begin{minted}[
    bgcolor=backcolor,
    frame=lines,
    framesep=1mm,
    % baselinestretch=1.2,
    fontsize=\tiny,
    linenos,
    numbers=right,
    % baselinestretch=.93,
    breaklines
]{python}
import torch
import torch.nn.functional as F

def fused_forward(self, feature, style):
    """
    feature: Feature with shape (B, C1, H, W)
    style  : Fusion style with shape (B, C2, H, W)
    """
    batch, in_c, in_h, in_w = feature.shape
    st_c = style.shape[1]
    
    # Hyperparameters
    k = self.kernel_size # Conv kernel size
    out_c = self.out_c   # Expected output channel
    rmpad = k // 2       # Zero-padding removal

    # Weight scaling (StyleGAN2)
    # Shape:
    # (1, ) * (out_c, in_c, k, k)
    # => (out_c, in_c, k, k)
    weight = self.scale * self.weight

    # Weight modulation (Casted)
    #   The following two forms are equivalent:
    #    - conv(in=feature,       w=weight*style*demod)
    #    - conv(in=feature*style, w=weight) * demod
    #   StyleGAN2 uses the former one for speed.
    style = \
        style.permute(0, 2, 3, 1).reshape(-1, st_c)
    style = self.modulation(style)
    style = style.view(batch, in_h, in_w, in_c)
    style = style.permute(0, 3, 1, 2)
    feature = (style * feature) # (B, C, H, W)

    # Weight demodulation (Approximated)
    #   Feature demodulation use patch statistics.
    #   The approximation here is similar to a 
    #   mean of statistics from all styles.
    demod = torch.zeros(batch, out_c, in_h, in_w)
    for i in range(in_h):
        for j in range(in_w):
            style_v = style[:, :, i, j] \
                .view(batch, 1, in_c, 1, 1)
            style_v = weight.unsqueeze(0) * style_v
            # style_v shape: (B, out_ch, in_ch, k, k)
            demod[:, :, i, j] = \
                torch.rsqrt(
                    style_v.pow(2).sum([2,3,4]))

    # Convolution
    # (All feature uses same weight, no need to group)
    if self.upsample:
        weight = weight.view(out_c, in_c, k, k)
        weight = weight.transpose(0, 1).contiguous()
        out = F.conv_transpose2d(
            feature, weight, 
            padding=0, stride=2, groups=1)


        # Clipping zero padding (ConvT special case)
        out = out[:, :, rmpad:-rmpad, rmpad:-rmpad]

        # Late demodulation (match output shape)
        demod = F.interpolate(
            demod,
            size=(out.shape[-2], out.shape[-1]),
            mode="bilinear", align_corners=True)
        out = out * demod

        out = self.blur(out) # StyleGAN2 Gaussian blur
    else:
        out = F.conv2d(
            feature, weight, padding=0, groups=1)
        demod = demod[:, :, rmpad:-rmpad, rmpad:-rmpad]
        out = out * demod
        
    out = out.contiguous()


    return out
\end{minted}

==> codes/scaleinv_fid.tex <==
\begin{minted}[
    bgcolor=backcolor,
    frame=lines,
    framesep=1mm,
    % baselinestretch=1.2,
    fontsize=\footnotesize,
    linenos,
    numbers=left,
    % baselinestretch=.93,
    breaklines
]{python}
import torch.nn.functional as F

def eval_scaleinv_fid(real_imgs, fake_imgs, scale):
    # real_imgs: tensor of real images, shape (B, C, H, W).
    # fake_imgs: tensor of fake images, shape (B, C, H, W).
    # scale:     the scale of the current ScaleInv FID.
    fake_images = F.interpolate(
        fake_images, 
        scale_factor=1/scale, 
        mode="bilinear", 
        align_corners=True)
    
    # The regular FID evaluation
    return eval_fid(real_images, fake_images)
\end{minted}


